First survey of centimeter-scale AC-LGAD strip sensors with a 120 GeV proton beam

We present the first beam test results with centimeter-scale AC-LGAD strip sensors, using the Fermilab Test Beam Facility and sensors manufactured by the Brookhaven National Laboratory. Sensors of this type are envisioned for applications that require large-area precision 4D tracking coverage with economical channel counts, including timing layers for the Electron Ion Collider (EIC), and space-based particle experiments. A survey of sensor designs is presented, with the aim of optimizing the electrode geometry for spatial resolution and timing performance. Several design considerations are discussed towards maintaining desirable signal characteristics with increasingly larger electrodes. The resolutions obtained with several prototypes are presented, reaching simultaneous 18 micron and 32 ps resolutions from strips of 1 cm length and 500 micron pitch. With only slight modifications, these sensors would be ideal candidates for a 4D timing layer at the EIC.

==> OldText.tex <==
%The results presented in this paper is based on data samples of interactions with a \SI{120}{\GeV} proton beam collected for each AC-LGAD sensor individually at the FNAL test beam facility.

%The key components of the setup is the trigger, proton hit position reference, proton arrival time reference, and AC-LGAD's data acquisition electronics. 
%The FTBF provides the large scintillator based trigger and the silicon tracking telescope that measures the position reference of each incident proton.
%Further details of the experimental setup can be found in references, which presents the results of the 2020 and 2021 beam campaigns.


\begin{figure}[htp]
\centering
\includegraphics[width=0.99\textwidth]{pictures/FTBF_Diagram_2022.pdf}

\vspace{0.5cm}

\includegraphics[width=0.99\textwidth]{pictures/TestBeamPic2022.jpeg}
\caption{Diagram of the AC-LGAD and reference instruments along the beamline (top). The environmental chamber placed within the FTBF silicon telescope (bottom). The telescope comprises five pairs of orthogonal strip layers and two pairs of pixel layers, for a total of up to 14 hits per track. 
\label{fig:FTBF_Box}}
\end{figure} %FTBF_Box

% The data acquisition electronics used in this campaign is identical to the electronics used in the 2021 beam test, which includes the oscilloscope that digitized the signals from the AC-LGAD, the detector that proves the fast arrival time reference, and the sensor mounted readout board.
% The Lecroy Waverunner 8208HD oscilloscope features eight readout channels with a bandwidth of \SI{2}{\giga \hertz} and a sampling rate of \SI{10}{GS/s} per channel. 
% The AC-LGAD under study occupied seven readout channels, while the eighth was used for the Photek micro-channel plate detector (MCP--PMT) as a reference for the proton arrival time. The MCP--PMT time resolution for signals from protons has been measured to be about \SI{10}{\ps}. 
% The AC-LGAD sensors were mounted on the readout boards developed by Fermilab~\cite{HELLER2021165828} and optimized for LGAD sensors, capable of accommodating 16~independent channels. 

% The key changes from the last beam test setup in 2021 was the upgrades made to the FTBF tracking telescope by the facility managers, the trigger, and the alignment procedure of the sensor used during the analysis within the tracking telescope reference frame.
% The main motivation for these changes was to account for the increased size of the AC-LGAD sensors.

% The position resolution of the tracker telescope measurement at the AC-LGAD location will be about a factor of four times greater than the expected resolution of the AC-LGAD sensors.
% Thus, the contribution of the tracker telescope to the AC-LGAD position resolution will not be significant.
% The track reconstruction algorithm based on the Kalman filter provides an estimate of the impact parameter resolution for each track based on the compatibility of the track fit with the observed hits. 
% This yields an estimated resolution of roughly \SI{5}{\um}. 
% Since the Kalman filter resolution does not include contributions from the alignment with the device under test, we take its estimate as a lower bound and have made an effort to minimize the AC-LGADs alignment impact on the tracker telescope resolution.

% When defining the proton hit location on the AC-LGAD, the initial assumption is to define the AC-LGAD as a plane perpendicular to the beam line and the proton track as a line in the three dimensional space defined by the tracking telescope.
% Then, we can determine the proton hit location as the intersection of the line and plane for each incident proton.
% As a consequence, any deviation to the physical alignment of the AC-LGAD due to mechanical or mounting variations will contribute to the measured position resolution.
% The misalignment contribution can be accounted for by measuring the three angles of rotation and the overall position along the beam line axis of the plane within the tracking telescope coordinates. 
% We measured these four values for each sensor by computing the position resolution for a range of variations around the nominal position of all four variables. 
% For example, we assumed the angle corresponding to the alignment of the AC-LGAD plane with respect to the $x-y$-axis to be at zero degrees, so to account from deviations of this assumption we then compute the proton track line--plane intersection for a set of small deviations in this angle to determine the value that minimizes the overall position resolution. 
% We repeated this scan of all four variables one at a time until we found the nominal value for each variable. 
% With this well defined alignment procedure we can assume the sensor alignment contribution to the measured position resolution is negligible and allowed us to verify the use of the Kalman filter method for measuring the tracking telescope resolution. 

% For the AC-LGAD resolutions presented in all plots and figures in this paper, we subtract the contributions from the tracking telescope and MCP--PMT on the measurements. 
% This corresponds to a value of \SI{5}{\micro\m} and \SI{10}{\ps} subtracted in quadrature for the position and time resolution respectively. 
